Learning to Represent Human Motives for Goal-directed Web Browsing

Motives or goals are recognized in psychology literature as the most fundamental drive that explains and predicts why people do what they do, including when they browse the web. Although providing enormous value, these higher-ordered goals are often unobserved, and little is known about how to leverage such goals to assist people's browsing activities. This paper proposes to take a new approach to address this problem, which is fulfilled through a novel neural framework, Goal-directed Web Browsing (GoWeB). We adopt a psychologically-sound taxonomy of higher-ordered goals and learn to build their representations in a structure-preserving manner. Then we incorporate the resulting representations for enhancing the experiences of common activities people perform on the web. Experiments on large-scale data from Microsoft Edge web browser show that GoWeB significantly outperforms competitive baselines for in-session web page recommendation, re-visitation classification, and goal-based web page grouping. A follow-up analysis further characterizes how the variety of human motives can affect the difference observed in human behavioral patterns.

==> sections/relatedWork.tex <==
% Bahar: Adding related work to support different claims

\section{Browsers and Interruption to Goal Pursuit}
- research on work vs life tasks in the online world:

As more and more work and personal activities take place online,
the separation between workers’ personal and professional
spheres is disappearing \cite{tseng2019overcoming}. In fact, personal internet usage while at work is common, with workers reporting spending 51 minutes on average over a workday in a 2012 study \cite{lim2012cyberloafing}.

Prior research has shown that workers experience
difficulty when resuming their main task after an external- or
self-interruption \cite{gillie1989makes, mcfarlane2002scope, o1995timespace} and thus might seek a diversion to a distracting website. In particular, self-interruptions
account for 40\% of interruptions \cite{czerwinski2004diary} and may be more
disruptive than external interruptions \cite{adler2013self}.

- research on Cyberloafing:

Epstein et al. \cite{epstein2016taking} identified that resuming work after a break can often
be difficult if the worker does not feel ready to work. As
a result, workers will often engage in non-work-related
online activities when they return to their desk (e.g., reading
news, checking personal email, browsing Facebook) rather
than engaging in work tasks, potentially leading to a "chain
of diversions" \cite{iqbal2007disruption} and ``Cyberloafing'' — defined as the
voluntarily use of digital technologies for non-work purposes
during working hours \cite{glassman2015monitor, lim2002way}.
One approach for combating cyberloafing is to block
access to non-work sites altogether. However, preventing
workers from taking digital breaks is inadvisable, as recent
studies have pointed to the importance of digital breaks
for combating boredom \cite{pindek2018cyberloafing}, increasing productivity \cite{epstein2016taking},
and for managing the work/life balance and reducing stress
\cite{anandarajan2005developing}. Another approach controls access to non-work sites
but relies on the worker to self-regulate their break-taking
behavior.

- research on technology distractions in education which is relevant to use of Internet in classroom:

Previous research on distractions and the use of mobile devices (personal digital assistants, tablet personal computers, or laptops) have been conducted almost exclusively in higher education.
Research on the distraction caused by technology in the classroom is relevant. 
For example, In 2003, researchers (Hembrooke & Gay, 2003) of Cornell
University conducted research into distraction of Information and Communication Technology (ICT) devices in the classroom. In an experiment, they divided a class of students into two groups. 
One group was allowed to use computers, connect to the Internet and
browse the web while attending a lecture. The other group attended the same
lecture, but was not allowed to use computers. A log of the activity of the group of
students with the computer showed that they looked at sites related to the lecture
but also visited unrelated sites, checked their emails, shopped online, watched
videos and did all the other things that people do online. Immediately after the
lecture both groups took a test measuring how well they could recall the
information from the lecture. The web surfers “performed significantly poor on
immediate measures of memory for the to-be-learned content of the lecture”,
according to researchers. 

General research on interruption and multi-tasking is relevant.
For example, Nicholas Carr, author of “The Shallows: What the Internet is Doing to Our
Brains”, argues that psychological research long ago proved what most of us know
from experience: frequent interruptions scatter our thoughts, weaken our memory,
and make us tense and anxious. The more complex the train of thought we are
involved in, the greater the impairment the distraction causes. Depending on the
how many information streams we subscribe to and the frequency with which they
send out updates, we may field a dozen alerts an hour, and for the most connected
amongst us, the number can be much higher. Each of them is a distraction, another
intrusion on our thoughts, another bit of information that takes up precious space
in our working memory.(Carr, 2010).

Every time we shift our attention, our brain has to reorient itself, further
taxing our mental resources. According to (Jackson, 2008) in her book, Distracted
that focuses on multitasking, “the brain takes time to change goals, remember the
rules needed for the new task, and block out cognitive interference from the previous,
still-vivid activity. Many studies have shown that switching between just two tasks can
add substantially to our cognitive load, impeding our thinking and increasing the
likelihood that we will overlook or misinterpret simple information.


-------------------------------------------------------------------------------------
Characterizing Online Browsing Behavior --> Multitude of activities accommodated by the Browsers

Since the inception of the World-Wide Web some fifteen years ago, the rate of appearance of new capabilities, data types, and services has remained high, allowing users to meet more of their communications, entertainment, and task completion needs online. Every day, new websites appear, exploring new approaches and business models in competition with existing online and offline alternatives. Hundreds of millions of users engage daily with social networking sites that offer capabilities that were unknown just a few years ago. 
Search of webpages, videos, images, commercial listings, personal ads and so forth continues to grow in volume and sophistication. 
Users engage with the offerings afforded by this crucible, and their behavior evolves as rapidly as the business landscape underlying it. 
This evolution, however, is difficult to observe, partly because of its velocity and partly because user behavioral data is not generally available for study. Thus, we lack an accurate picture of how users engage with the Web.

A a new CCS taxonomy of pageviews consisting of Content (news, portals, games, verticals, multimedia), Communication (email, social networking, forums, blogs, chat), and Search (Web search, item search, multimedia search) was proposed in 2010. 
Kumar and Tomkins showed that show that roughly half of all pageviews online are content, one-third are communications, and the remaining one-sixth are search. 


==> sections/s1_introduction.tex <==
\section{Introduction}
\label{section:introduction}

Web browsers play a critical role in our personal and work lives --- they serve as a gateway to the open web and help people pursue and complete their diverse goals, such as productivity, wellbeing, personal growth, etc.~\cite{taivalsaari2008web}. \bs{I strongly suggest considering changing this paragraph based on Jaime's comment on the WWW paper. See comments.} \longqi{Yes, Bahar, please go ahead and change it, and if you can, also update the abstract and make it consistent}
%the browser has become a fully-functional operating system in the cloud era~\cite{taivalsaari2008web}.    
%The diversity and comprehensiveness of browsers, while providing indispensable value, can create challenges for people who interact with them. 
However, studies have shown that people are often unable to focus on or return to their goals when using a web browser due to the prevalence of distractions on the web~\cite{aagaard2015drawn, tseng2019overcoming}. For example, XXXX \longqi{Bahar/JJ, Can you find several citations to back this up? and also give an example study/statistic}.\bs{I added a relatedWork.tex file to collect a bunch of references. They are mostly on this concept of *CyberLoafing*. I'll add a few sentences here once I'm done.} 
% This is particularly challenging when returning to a previously unfinished goal, since people may need to spend time retrieving relevant resources and reminding themselves of where they were.   

%\bs{Before this paragraph we need a framing sentence that clarifies there are two main paradigms of activities that are commonly supported by modern browsers: Search (by query) and more general browsing and visiting Web pages. Supporting search goals is a well-studied problem in the IR community ... all references ... But searching is only a portion of activities on the Browser ... continuing with supporting more general browser activities.}
%\jj{fixed the issue.}
\new{User behaviors using modern web browsers can be simply categorized into two types, including \textit{web search} (e.g., submitting queries and clicking search results) and \textit{general web browsing} (e.g., visiting web pages with URLs and booklets)}.
To address this problem \new{for web search}, prior work~\cite{broder2002searchtaxonomy,CARUCCIO2015userintent,rose2004usergoal,Uichin2005} has sought to categorize the intents or goals behind search queries to understand what people want to achieve. 
In their seminal works, Broder~\cite{broder2002searchtaxonomy} and Rose and Levinson \cite{rose2004usergoal} classified the goal of a user query into one of three categories: navigational, informational, and transactional.
%Following this canonical taxonomy, subsequent studies have investigated ways to building predictive models \cite{CARUCCIO2015userintent} or adding sub-classes as an enrichment \cite{CARUCCIO2015userintent}.
For more complex search needs, research~\cite{jones2008searchtopics, Law2011complexsearch} has shown that identifying coherent intents algorithmically across queries or sessions can help satisfy people's needs faster. 
Compared to search which comprises only about one-sixth of browser activities~\cite{kumar2010browsing}, general web browsing patterns tend to involve significantly higher complexity.
Prior work introduced a program-by-example goal-oriented web browser~\cite{Faaborg2006AGW} that allows people to customize rules to extract useful information across similar websites (e.g., nutrition from recipe websites), as well as an interactive summary of browsing sessions \cite{Dontcheva2006Summarizing} for easier resumption of encountered entities.


However, existing methods can be myopic as they are mostly focused on short-term tasks.
We argue that considering long-term goals is crucial for intelligent web browsers, as they are influential to the fundamentals of human behavior~\cite{Chulef2001AHT}; for instance, goals such as \textit{staying healthy} or \textit{having personal growth} serve a directional role that impacts our everyday thoughts and actions. 
With the ability to model long-term goals, browsers can bring substantial benefits to people's lives \cite{Barua2014longtermgoals} including health, well-being, sustainability and learning.


ㄎIn this paper, we propose an unified framework, \modelfullname~(\modelname), that allows browsers to understand and leverage people's long-term goals (Figure~\ref{fig:overall}). Specifically, \modelname builds generic goal-aware representations (both in-session and long-term) by integrating goal representations learned in a hyperbolic space with BERT~\cite{devlin2019bert}-based text representation. We then leverage these enriched representations to improve three intelligent browser functionalities: (1) in-session web page recommendation aiming to recommend web pages that can help advance people's goals in each session, (2) web page re-visitation classification that predicts if a person will revisit a web page in the future due to recurring or unfinished goals, and (3) goal-based web page grouping that clusters in-session web pages according to underlying goals.

% Based on given goal representations of web page visits, \modelname enriches the text understanding capability of BERT~\cite{devlin2019bert} by not only integrating the in-session contextualized goals via multi-headed attention~\cite{NIPS2017_7181}, but also attending~\cite{vaswani2017attention} to each individual's preferences in the goal space.
% Specifically, the recommendation task aims to recommend web pages that can help advance people's goals in each session. 
% The revisitation classification task predicts if a person will revisit a web page in the future potentially due to recurring or unfinished goals. The grouping task focuses on clustering in-session web pages by the goals that drive people performing the visits.

As a critical component of \modelname, we propose a novel approach for goal representation learning as shown in Figure~\ref{fig:overall}.
Inspired by psychology literature, we leverage a representative human long-term goal taxonomy \cite{Chulef2001AHT} where a goal is defined as subjectively desirable future states of affairs that an individual intends to attain through actions \cite{Moskowitz2009ThePO}. 
This taxonomy allows us to capture open-domain web browsing goals beyond web search. To retain the hierarchical relationship between goals (e.g., the goals ``be affectionate'' and ``share feelings'' are both decedents of ``friendship''), we design a structure-preserving strategy to learn goal representations in a hyperbolic space. Using a weak supervision approach, we further introduce a goal estimator to predict the goals that an individual may have when visiting a web page. 
% This way, the unobserved property of how people pursue their goals can be associated with the observed web browsing flows. 
%\longqi{This paragraph needs to go to somewhere else}
Moreover, to overcome some of the previous challenges in coverage and scalability, we leverage large-scale pre-trained language models \cite{devlin2019bert} to associate human goals with atomic informational units in browsers, i.e., web pages, instead of search queries. By doing so, we enable the generality of modeling capability, which in turn can facilitate diverse downstream applications. 



\if 0

We propose a two-phase process as illustrated in Figure~\ref{fig:overall}. The first phase targets learning human goal representations. Taking a psychology perspective, we leverage a representative human long-term goal taxonomy curated by \citet{Chulef2001AHT}, where a goal can be understood as subjectively desirable future states of affairs that an individual intends to attain through actions \cite{Moskowitz2009ThePO}. 
The adoption of human goals facilitates capturing the greatest common denominator in open-domain web browsing, beyond just search goals. 
Specifically, we employ a structure-preserving strategy for learning goal representations in a hyperbolic space, in a way that the hierarchical relation between goals can be retained\footnote{E.g., The goals ``be affectionate'' and ``share feelings'' are both decedents of ``friendship''.}. 
Using a weak supervision approach, we further introduce a goal estimator that is trained to predict which goals of an individual may have driven their visits to certain web pages. This way, the unobserved property of how people pursue their goals can be associated with the observed web browsing flows. 
%we learn to project arbitrary web pages into the same hyperbolic space, effectively associating human goals and browsing information flows.    

Building on the goal representations, the second phase presents a deep neural framework to incorporate such goal awareness into three browser-centric tasks, as shown Figure~\ref{fig:overall}.  
The unified framework, \modelfullname~(\modelname), enriches the text understanding capability of BERT~\cite{devlin2019bert} by not only integrating the in-session contextualized goals via multi-headed attention~\cite{NIPS2017_7181}, but also attending~\cite{vaswani2017attention} to each individual's preferences in the goal space.
Specifically, the recommendation task aims to recommend web pages that can help advance people's goals in each session. 
The revisitation classification task predicts if a person will revisit a web page in the future potentially due to recurring or unfinished goals. The grouping task focuses on clustering in-session web pages by the goals that drive people performing the visits.

\fi 

%, and identifies potential distractions via modeling``non-goals''. 

We evaluate \modelname using anonymized browsing logs obtained from the Microsoft Edge browser.   
The experimental results show that \modelname consistently outperforms competitive baselines in all three downstream tasks, suggesting that capturing fundamental human motives can significantly improve the intelligence of web browsers.
%modeling human goals in web search sessions can benefit a variety of useful applications.
%Our follow-up analysis further sheds light on how different goals might impact people's browsing behavior differently.
Our followup analysis further demonstrates that our learned hyperbolic goal embeddings largely preserve the human-curated hierarchical relations; meanwhile, the goal estimator is effective in deriving goal representations for web page visits.
Besides, people may pursue interleaved goals when a goal has a broad meaning (e.g., \textit{Ethics \& Idealism}), while they may revisit web resources faster for goals concerning social interactions (e.g., \textit{Friendship})

%\longqi{This seems out of the blue. What do we want to convey here?}
%Besides, people may pursue interleaved goals when a goal has a broad meaning (e.g., \textit{Ethics \& Idealism}), while they may revisit web resources faster for goals concerning social interactions (e.g., \textit{Friendship})

%\longqi{I have done a pass of the intro.}
%Our follow-up analysis further sheds light on how different goals that drive visits to web pages might impact browsing behavior differently.
%Moreover, in-depth analysis also justifies our motivation and gives several insights about human goals in web browsing behaviors. 

%\vspace{-9pt}

==> sections/sz_backup_goal_estimator_eval.tex <==
\if 0
\subsection{Goal Estimator Performance}
\label{sec:goalestimatorperf}
\input{tables/goalestimator}

\input{tables/misclassification}

\input{tables/tophost}

Recall that the goal estimator is learned with a multi-class objective, where a 136-way classification is carried out to predict among the 135 leaf goals in the taxonomy plus a non-goal class.  
We use 90\% of weakly-labeled instances from $\bm{D}_{weak}$ for training, and evaluate on the remaining 10\% with standard metrics including accuracy and macro/micro F1 scores.
%To evaluate its performance, we 
%We train the goal estimator using 90\% of weakly-labeled instances from $\bm{D}_{weak}$ and evaluate on the remaining 10\% 
%with goal classification based on the weakly-labeled dataset mentioned in Section~\ref{fig:goal_estimator}. 
%\cj{worth reminding readers of the data in sec 3 again.}
%Specifically, we evaluate the predicted goals $g_p$ with the ground truth goals $\hat{g}_p$.
% \cj{isn't the convention usually that hat means prediction?}
%Here we treat the task as a 135-way classification problem to identify 135 goals in the taxonomy and evaluate the performance with conventional metrics, including the accuracy and macro/micro F1 scores.
%Note that ``non-goal'' presents empty prediction of goals and only affects the recall but precision.
Table~\ref{tab:goalestimator} shows the classification performance of the goal estimator. %\cj{here we don't have \modelname yet? \modelname I thought is for sec 4?}
Considering that a random classifier predicts with an expected accuracy of 1/136=0.73\%, our goal estimator performs reasonably with 58.81\% accuracy and 55.27\% Micro-F1 score.
We further conduct an ablation analysis to study the effectiveness of the neural blocks in the web page encoder illustrated in Figure~\ref{fig:wegbpage_encoder}.
Table~\ref{tab:goalestimator} suggests that modeling web page content is key to the overall performance, and the ensemble of two sources achieves the best results.
%It shows that the goal estimator is capable of interpreting the goals behind web pages with learned goal embeddings.
%The ablation study indicates most of the gains are from modeling contents, whereas hosts can be useful in the ensemble of two resources.
%Moreover, it shows that identifying goals behind web pages is a difficult task that cannot be solely solved by the website information.

Since the accuracy scores are not exactly perfect, we conduct analysis on the predictions to better understand where the model fails.
Figure~\ref{fig:goal_heat_map} depicts the confusion matrix for our goal estimator, where the grid partitions leaf goals into goal categories.
We can see that most of the predictions are aligned with the diagonal as correct predictions; among other cases, most of the misclassifications are in the same category, i.e., the same block in the grid. %\cj{how to read categories from the figure -- I guess need to explain the grids a litte more.}
Examining the top misclassifications, we show in Table~\ref{tab:misclassification} that most of the misclassifications are semantically similar to the actual goals and could belong to the same goal category.
For instance, the examples 1 to 4 indicate that some goals under the same category can be very similar. %\cj{Do we have a category level accuracy/pre/recall?}
The example 5 additionally shows that the goal estimator may classify web pages pertaining to a broader goal into similar, more specific goals.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\linewidth]{img/goal_heat_map.eps}
    \caption{The probabilistic confusion matrix for our goal estimator in goal classification. The grid partitions goals into categories. The ``non-goal'' class has goal ID 1.}
    \label{fig:goal_heat_map}
\end{figure}


We further conduct a lightweight qualitative exercise to analyze the relations between hosts and predicted goals. 
%We further analyze the relations between hosts and predicted goals behind their web pages.
We first identify top hosts that cover a higher proportion of web pages being predicted closest to each goal category.
Two annotators were then asked to judge whether these hosts are relevant to the corresponding categories.
Table~\ref{tab:tophost} shows the assessment results with 100\% agreement from the two annotators.
%Table~\ref{tab:tophost} lists the top hosts with a higher coverage of web pages belonging to certain goal categories.
%Two annotators manually labeled if these hosts are relevant to the corresponding categories with 100\% agreement.
The assessments suggest that the goal estimator can make reasonable predictions in the majority of cases.  
%most of the top hosts are related to the goals in the categories and also demonstrate the effectiveness of our proposed goal estimator.
For goals of high specificity, such as  \textit{Career} and \textit{Religion}, we find that the goal estimator can effectively identify websites designated for the corresponding purposes.   
The predictions tend to be less precise when a goal can be pursued in many ways; for example, encyclopedia and news websites are predicted to be associated with \textit{Entertainment}.


%For the goals with more specific purposes, such as  \textit{Career} and \textit{Religion,} there would be more websites that majorly consist of web pages matching a certain goal.
%On the contrary, the goals like \textit{Entertainment} with diverse concepts and no strong focus, users may tend to browse web pages in comprehensive resources, such as encyclopedia and news websites.


\fi 






==> tables/goalestimator.tex <==
\begin{table}[!t]
    \centering
    \begin{tabular}{c|ccc} \hline
    	 & Accuracy	& Macro-F1	& Micro-F1 \\\hline
Goal Estimator & 0.5881 & 0.4275 & 0.5527 \\\hline
Contents Only & 0.5316 & 0.3689 & 0.4914 \\
Host Only & 0.1140 & 0.0154 & 0.0367  \\ \hline
    \end{tabular}
    \caption{Classification performance of the full-versioned goal estimator, as well as ablated versions that use only the content or host neural blocks.}
    \label{tab:goalestimator}
\end{table}

==> tables/misclassification.tex <==
\begin{table*}[!t]
    \centering
    \resizebox{.95\linewidth}{!}{
    \begin{tabular}{|c|p{.45\linewidth}|p{.45\linewidth}|} \hline
        Example &  Actual Goal (Category) &  Mispredicted Goal (Category) \\ \hline \hline
        1 & Having a stable, secure family life (Family) &  Feeling close to my parents, siblings, grandparents  (Family) \\\hline
        2 & Being close to my spouse (Marriage) & Having a good marriage (Marriage)\\ \hline
        3 & Being creative (Creativity) & Having original, novel ideas (Creativity) \\ \hline
        4 & Achieving my aspirations (Achievement) &  Being ambitious, hard-working (Achievement) \\ \hline
          & \multirow{2}{*}{Providing my spouse or children (or both) with a feeling}  & Being close to my spouse (Marriage)\\
        5 & \multirow{2}{*}{of financial security and a home to come back to (Family)}  & Being a good parent  (Family)\\
          &  & Having a stable, secure family life (Family)\\ \hline
    \end{tabular}}
    \caption{Examples of top misclassifications for five goals in the goal estimator evaluation.}
    \label{tab:misclassification}
    \vspace{-12pt}
\end{table*}

